Free-rider Attacks on Model Aggregation in Federated Learning

Free-rider attacks against federated learning consist in dissimulating participation to the federated learning process with the goal of obtaining the final aggregated model without actually contributing with any data. This kind of attacks is critical in sensitive applications of federated learning, where data is scarce and the model has high commercial value. We introduce here the first theoretical and experimental analysis of free-rider attacks on federated learning schemes based on iterative parameters aggregation, such as FedAvg or FedProx, and provide formal guarantees for these attacks to converge to the aggregated models of the fair participants. We first show that a straightforward implementation of this attack can be simply achieved by not updating the local parameters during the iterative federated optimization. As this attack can be detected by adopting simple countermeasures at the server level, we subsequently study more complex disguising schemes based on stochastic updates of the free-rider parameters. We demonstrate the proposed strategies on a number of experimental scenarios, in both iid and non-iid settings. We conclude by providing recommendations to avoid free-rider attacks in real world applications of federated learning, especially in sensitive domains where security of data and models is critical.

==> tex/Background.tex <==
\section{Related Work}

\subsection{Federated Learning}

Federated Learning is a learning process with $I$ clients and a server $S$. Each client owns a private dataset with $M_i$ samples that cannot be shared.

In this setting, to fit a global model to this distributed dataset, FedAvg\cite{BrendanMcMahan2017} is based on the aggregation of model's parameters through an iterative averaging process. At each iteration $t$, the server sends the model parameters $\theta(t)$ to the clients participating in the training. Each client updates the model on $E$ epochs and sends back the updated local parameters $\theta_i(t)$ to the server that estimates the model parameters $\theta(t+1)$ as a weighted average of the local ones:
\begin{equation}
\label{FedAvg_server_aggregation}
\theta(t+1)=\sum_{i\in I}\frac{M_i}{N}\theta_i(t),
\end{equation}
where $N=\sum_{i\in I}M_i$ represents the total number of samples of the distributed dataset.




\subsection{Attacking Federated Learning}

Sharing the model parameters is shown to be less sensitive than sharing the dataset itself or the gradient but still sensitive XXX. Attacks can still be achieved against federated learning. Two types of attackers can be differentiated: active and passive.

\textbf{Passive attackers} can be considered as curious. The system integrity is respected. The attackers updates model according to the server directives. The attackers' aim is to have a better representation of the clients' data distribution: class representation XXX, data recovery XXX, membership attack XXX. Contrarily to the server, the clients only have access to the history of the aggregated models and therefore cannot attribute any retrieved information to a specific client.

\textbf{Active attackers} are ready to update any model to achieve their goal. When carried out by the server, these attacks aim at recovering the clients' data XXX. The server isolates each clients and generates for each of them a custom made model. The successive updates on the server generated model help the server recover samples from the client. However, when carried out by the clients, these attacks can have different goals: 1) Model Poisoning \cite{Fang2019,Bhagoji2019,LiDataPoisoning2016}. Compromised clients send back models misclassifying a set of chosen inputs with high confidence. (2) Byzantine Attack \cite{Yin2018,Fang2019,Bhagoji2019}. Active attackers send back to the server models that make the global model diverge. (3) Backdoor inclusion \cite{Bagdasaryan2018}. Attackers can return model performing well but with a backdoor that can last for a few iterations. (4) Data recovery \cite{Wang2019,Hitaj2017}. Attackers return to the server models that will force the fair clients to return to the server updated models revealing more information about the clients' dataset.



==> tex/broader_impact.tex <==
\section*{Broader Impact}

The problem of free-rider attacks in federated learning may have  significant economical and societal impact. Since it allows clients' participation without sharing the data, federated learning is becoming the de-facto training setup in current large-scale machine learning projects in several critical applications, such as healthcare, banking, and telecommunication. The resulting models derived from sensitive and protected data may have high commercial and intellectual value as well, due to their exclusive nature. Our research proves that if precautions are not taken, malicious clients can disguise their participation to federated learning to appropriate a federated model without providing any contribution. Our research therefore stimulates the investigation of novel verification techniques for the implementation of secured federated learning projects, to avoid intellectual property or commercial losses. 

% Authors are required to include a statement of the broader impact of their work, including its ethical aspects and future societal consequences. Authors should discuss both positive and negative outcomes, if any. For instance, authors should discuss a) who may benefit from this research, b) who may be put at disadvantage from this research, c) what are the consequences of failure of the system, and d) whether the task/method leverages biases in the data. If authors believe this is not applicable to them, authors can simply state this. Use unnumbered first level headings for this section, which should go at the end of the paper. Note that this section does not count towards the eight pages of content that are allowed.

==> tex/related_work.tex <==
\section{Related Work}

The study of security and safety of federated learning is an active research domain, and several kind of attacks have been studied. For example, an attacker may interfere during the iterative federated learning procedure to degrade/modify models performances\cite{Fang2019,Bhagoji2019,LiDataPoisoning2016,Yin2018,Bagdasaryan2018,Shen2016}, or retrieve information about other clients data\cite{Wang2019,Hitaj2017}.



%Not sharing the dataset itself with the master does not ensure complete privacy for the clients participating in a Federated Learning process. Different kind of attacks can be performed by malicious clients - attackers. By communicating to the master opportune results, the attackers can change the model performances or retrieve information about the other clients' datasets\cite{Wang2019,Hitaj2017}. 

%Sharing the model parameters enables a client to obtain a performing statistical model for an application with samples difficult to obtain. Yet, sharing the model parameters is only less sensitive than sharing the dataset itself or the gradient. Attacks can still be achieved against Federated Learning when the client or the master is curious, passive attack, or malicious, active attack.
%Sharing the model parameters is shown to be less sensitive than sharing the dataset itself or the gradient but still sensitive. Attacks can still be achieved against Federated Learning. Two types of attackers can be differentiated: active and passive.

%A passive attacker, while respecting the system integrity, aims at having a better representation of the clients' data distribution: class representation, data recovery, and membership attack. Instead, an active attacker is ready to update any model to achieve his goal. A malicious master or client can isolate each client and send them custom models forcing them to release more information about their dataset\cite{Wang2019,Hitaj2017}. However, a malicious client can also have different goals: (1) Model Poisoning \cite{Fang2019,Bhagoji2019,LiDataPoisoning2016}. Compromised clients update models misclassifying a set of chosen inputs with high confidence. (2) Byzantine Attack \cite{Yin2018,Fang2019,Bhagoji2019}. Attackers update models making the aggregated one diverge. (3) Backdoor inclusion \cite{Bagdasaryan2018}. Attackers update model performing well but including a backdoor.

%\textbf{Passive attackers} can be considered as curious. The system integrity is respected. The attackers update model according to the master directives. The attackers' aim is to have a better representation of the clients' data distribution: class representation, data recovery, and membership attack. Contrarily to the master, the clients only have access to the history of the aggregated models and therefore cannot attribute any retrieved information to a specific client.

%\textbf{Active attackers} are ready to update any model to achieve their goal. When carried out by the master, these attacks aim at recovering the clients' data. The master isolates each clients and generates for each of them a custom made model. The successive updates on the master generated model help the master recover samples from the client. However, when carried out by the clients, these attacks can have different goals: (1) Model Poisoning \cite{Fang2019,Bhagoji2019,LiDataPoisoning2016}. Compromised clients update models misclassifying a set of chosen inputs with high confidence. (2) Byzantine Attack \cite{Yin2018,Fang2019,Bhagoji2019}. Attackers update models making the aggregated one diverge. (3) Backdoor inclusion \cite{Bagdasaryan2018}. Attackers update model performing well but with a backdoor lasting for a few iterations. (4) Data recovery \cite{Wang2019,Hitaj2017}. Attackers update models forcing the fair clients to update models revealing more information about their dataset.

==> tex/removed.tex <==
\subsection{Experiment 2: Comparing the Server Model over time with one freeloader and changing the number of owned samples by freeloader}


We redo the same experiment with different number of samples owned by the freeloader: mean number of samples, maximum participating number of samples, and two times the maximum. In the different learning settings, we use $p=0.2$ and $\gamma=0.1$ for the additive, multiplicative and combination of the two noises. 
\begin{figure}
	\begin{subfigure}{.3\textwidth}
		\centering
		%\includegraphics[width=3cm,height=3.5cm]{example-image-a}
		\caption{additive noise}
	\end{subfigure}\hfill
	\begin{subfigure}{.3\textwidth}
		\centering
		%\includegraphics[width=3cm,height=7cm]{example-image-b}
		\caption{multiplicative noise}
	\end{subfigure}\hfill
	\begin{subfigure}{.3\textwidth}
		\centering
		%\includegraphics[width=3cm,height=7cm]{example-image-c}
		\caption{additive+multiplicative noise}
	\end{subfigure}
	\caption{Test on the influence of the number of samples on the convergence speed with only one freeloader}
	\label{diff_number_samples_one_freeloader}
\end{figure}

Expecting results: the more data the freeloader pretends having the slower the convergence. \ref{diff_number_samples_one_freeloader}

\textbf{Might be an useless experiment considering experiment 3 is a generalization of this one.}



\subsection{Experiment 3:Influence of the system integrity on the convergence speed}

We add $x$\% of clients to the original dataset where $x\in [1,5,10,20,50]$. Each freeloader pretends having the average number of samples. We consider different noise type, additive, multiplicative and a combination of the two. For all the freeloaders, $p=0.2$ and $\gamma_i=0.1$. \\
\textbf{We could alternatively give different standard deviation for each freeloader and sample their standard deviation uniformly}

\begin{figure}
	\begin{subfigure}{.3\textwidth}
		\centering
		%\includegraphics[width=3cm,height=3.5cm]{example-image-a}
		\caption{additive noise}
	\end{subfigure}\hfill
	\begin{subfigure}{.3\textwidth}
		\centering
		%\includegraphics[width=3cm,height=7cm]{example-image-b}
		\caption{multiplicative noise}
	\end{subfigure}\hfill
	\begin{subfigure}{.3\textwidth}
		\centering
		%\includegraphics[width=3cm,height=7cm]{example-image-c}
		\caption{additive+multiplicative noise}
	\end{subfigure}
	\caption{Influence of the ratio of data owned by the freeloaders on the convergence speed}
	\label{diff_number_samples_many_freeloader}
\end{figure}

Expecting results: the more data the freeloaders pretend having the slower the convergence. \ref{diff_number_samples_many_freeloader}




\subsection{Experiment 4: Freeloaders detection by the server}

We consider a learning process with 30\% of the clients that are freeloaders all having linear processes $f_i$. The server is looking for freeloaders with a linear noise model $f$. So $f$ and $f_i$ are linear functions. 10\% of the freeloaders have an additive noise model. 10\% a multiplicative noise and the remaining 10\% a combination of the two. Each 10\% will be divided into 4 groups of different standard deviation: $p\in[0.05,0.1,0.2,0.5]$ with $\gamma=0.1$ for all the clients. We consider that if the metric for a client after 3 consecutive iterations is under $10^{-3}$ then the client would have been detected a freeloader and been removed of the learning process. We therefore still continue the training with the detected freeloaders. The server only start looking for freeloaders after 10 iterations. 

\iffalse
\begin{figure}
	\begin{subfigure}{.3\textwidth}
		\centering
		%\includegraphics[width=3cm,height=3.5cm]{example-image-a}
		\caption{additive noise}
	\end{subfigure}\hfill
	\begin{subfigure}{.3\textwidth}
		\centering
		%\includegraphics[width=3cm,height=7cm]{example-image-b}
		\caption{model evolution}
	\end{subfigure}\hfill
	\begin{subfigure}{.3\textwidth}
		\centering
		%\includegraphics[width=3cm,height=7cm]{example-image-c}
		\caption{detection numbers}
	\end{subfigure}
	\caption{Number of detected freeloaders at each iteration since the beginning of the learning process}
	\label{server_detection}
\end{figure}
\fi

Expecting results: see the noise structures that are detected the fastest and see the percentage of participating clients detected as freeloaders. \ref{server_detection}
